Online Policy Optimization in Unknown Nonlinear Systems

We study online policy optimization in nonlinear time-varying dynamical systems where the true dynamical models are unknown to the controller. This problem is challenging because, unlike in linear systems, the controller cannot obtain globally accurate estimations of the ground-truth dynamics using local exploration. We propose a meta-framework that combines a general online policy optimization algorithm ($\texttt{ALG}$) with a general online estimator of the dynamical system's model parameters ($\texttt{EST}$). We show that if the hypothetical joint dynamics induced by $\texttt{ALG}$ with known parameters satisfies several desired properties, the joint dynamics under inexact parameters from $\texttt{EST}$ will be robust to errors. Importantly, the final policy regret only depends on $\texttt{EST}$'s predictions on the visited trajectory, which relaxes a bottleneck on identifying the true parameters globally. To demonstrate our framework, we develop a computationally efficient variant of Gradient-based Adaptive Policy Selection, called Memoryless GAPS (M-GAPS), and use it to instantiate $\texttt{ALG}$. Combining M-GAPS with online gradient descent to instantiate $\texttt{EST}$ yields (to our knowledge) the first local regret bound for online policy optimization in nonlinear time-varying systems with unknown dynamics.

==> proof_outline.tex <==
\subsection{Local Regret of OGD}

\begin{definition}[Projected gradient]
Let $F: \Theta \to \mathbb{R}$ be a differentiable function on a closed convex set $\Theta \subseteq \mathbb{R}^d$. For $\eta > 0$, the $(\Theta, \eta)$-projected gradient of $F$ is defined as
\[\nabla_{\Theta, \eta}F(\theta) \coloneqq \frac{1}{\eta}\left(\theta - \Pi_\Theta(\theta - \eta \nabla F(\theta))\right).\]
\end{definition}

\begin{theorem}\label{thm:nonconvex-biased-OGD}
Consider the parameter sequence $\{\theta_t\}$ that satisfies
\[\norm{\theta_{t+1} - (\theta_t - \eta \nabla_{\Theta, \eta}F_t(\theta_t))} \leq \eta \beta_t, \text{ for all }t \geq 0.\]
Suppose at every time $t$, $F_t$ is $\ell_F$-smooth and $L_F$-Lipschitz in $\Theta$. If the learning rate $\eta \leq \frac{1}{\ell_F}$, then the local regret $\sum_{t = 0}^{T-1}\norm{\nabla_{\Theta, \eta} F_t(\theta_t)}^2$ is upper bounded by
\begin{align*}
    &\frac{1}{\eta (1 - \eta \ell_F)}\left(F_0(\theta_0) + \sum_{t=1}^{T-1}\dist_s(F_t, F_{t-1})\right) + \frac{L_F \sum_{t=0}^{T-1} \beta_t + \ell_F \eta \sum_{t=0}^{T-1} \beta_t^2}{1 - \eta \ell_F},
\end{align*}
where $\dist_s(F, F') \coloneqq \sup_{\theta \in \Theta} \abs{F(\theta) - F'(\theta)}$.
\end{theorem}

\subsection{Adaptive Control}

\yiheng{Rather than adaptive control, I think we can also understand this as an online regression problem.}

\subsubsection{Online Parameter Estimation}

We first consider the case where the adaptive controller can make a noisy observation $(x_t, y_t)$ at time step $t$ that satisfies $x_t$ is bounded and
\[y_t = f_t(x_t, a_t^*) + v_t,\]
where $v_t$ is a random noise that is uniformly bounded and satisfies $\mathbb{E}\left[v_t\mid \mathcal{F}_t\right] = 0$, where the filtration $\mathcal{F}_t = \sigma(x_{0:t}, y_{0:t-1})$. A critical difference with standard (offline) regression problem is that $x_{t+1}$ can adapt to the sampling history.

At each time step, the agent decides $\hat{a}_t \in D$ before the data point $(x_t, y_t)$ is revealed. We require the adaptive controller (or online parameter estimation) to achieve the following guarantee:

\begin{theorem}[Meta]\label{thm:meta-online-param-est}
Suppose the sequence of exact predictions $\{a_t^*\}$ is oblivious and satisfies the path length constraint $\sum_{t=1}^{T-1} \norm{a_t^* - a_{t-1}^*} \leq C_p$. Then, the trajectory of the adaptive controller satisfies that $f_t(x_t, \hat{a}_t)$ is uniformly bounded and
\begin{align*}
    &\sum_{t=0}^{T-1} \norm{f_t(x_t, \hat{a}_t) - y_t}^2 - \sum_{t=0}^{T-1} \norm{f_t(x_t, a_t^*) - y_t}^2\\ \leq{}& R(T, C_p).
\end{align*}
\end{theorem}

\yiheng{The Meta Theorem is formulated based on the regret bounds derived in \cite{baby2021optimal} and our previous work \cite{lin2023online} (Theorem E.1).}

Note that \Cref{thm:meta-online-param-est} implies
\[\mathbb{E}\left[\sum_{t=0}^{T-1} \norm{f_t(x_t, \hat{a}_t) - f_t(x_t, a_t^*)}^2\right] \leq R(T, C_p).\]
Bounding the expected total squared distance of the gradients is more challenging. Define filtration $\mathcal{F}_t' = \sigma(x_{0:t}, y_{0:t})$. We provide a sufficient condition about the randomness on the dynamical system in 

\begin{assumption}\label{assump:perturb-the-state}
There is a certain level of random disturbances on the state $x_t$, i.e., one can find a $\sigma$-algebra $\mathcal{G}_t$ such that $\mathcal{F}_t' \subseteq \mathcal{G}_t \subseteq \mathcal{F}_{t+1}$ and
\begin{align*}
    \norm{x_{t+1} - \mathbb{E}[x_{t+1}\mid \mathcal{G}_t]} &\leq \overline{\sigma},\\
    \text{Cov}(x_{t+1} \mid \mathcal{G}_t) &\succeq \underline{\sigma} I.
\end{align*}
\end{assumption}
